STAGE: Diagnosing Semantic Transfer at Grounded Execution in Embodied Agents

Embodied language grounding requires more than identifying the referent of an instruction: recovered semantics must also control the action an agent exposes. We study this missing link as a semantic-action gap, where instruction semantics are recoverable but weakly expressed in native continuous actions. We introduce SAT-Bench, a fixed-observation counterfactual benchmark that holds the visual scene and agent state fixed while changing only instruction semantics. On LIBERO target-name and pixel-grounded relation swaps, target recovery reaches 100.0% and 95.8%, whereas OpenVLA action sensitivity remains only 6.8% and 7.7%. The gap persists across 1,000 additional compositional and temporal/procedural counterfactuals, with overall action sensitivity of 6.1%. Hidden-state, threshold-free, cross-policy, and rollout diagnostics further support this semantic-action transfer failure. We introduce VISA, a lightweight execution-time interface that converts recovered semantics into ALLOW, DEFER, target-consistency, and verified-selection decisions. VISA reduces invalid-instruction blind execution from 92.7% to 2.8% while preserving 94.0% of normal commands, and verified selection further improves target-consistent action exposure without updating the underlying policy. Overall, embodied language evaluation should measure semantic-action transfer, not semantic parsing alone.

==> sections/00_abstract.tex <==
\begin{abstract}
% Embodied language grounding requires more than recovering the referent of an instruction: recovered semantics must also control the action an agent exposes. We study this missing link as a \emph{semantic--action gap}, where instruction semantics are available but weakly expressed in native continuous actions. We introduce Semantic–Action Gap Framework, a fixed-observation counterfactual framework that holds the image and agent state fixed while changing only instruction semantics through controlled prompt transformations. On 600 LIBERO target-name swaps and 600 pixel-grounded relation swaps, a Qwen2.5-VL schema probe recovers the intended target in 100.0\% and 95.8\% of cases, yet OpenVLA action sensitivity is only 6.8\% and 7.7\%. We further introduce VISA, a lightweight, interpretable semantic-action interface that operationalizes recovered semantics as \textsc{allow}, \textsc{defer}, and target-consistency decisions, reducing invalid-instruction blind execution from 92.7\% to 2.8\% while preserving 94.0\% of normal commands. Across cross-policy, threshold-free, internal-probe, and short-horizon behavioral diagnostics, these results suggest that embodied language evaluation should test whether recovered semantics reach the action interface, not only whether they can be parsed.


Embodied language grounding requires more than identifying the referent of an instruction: recovered semantics must also control the action an agent exposes. We study this missing link as a \textbf{semantic–action gap}, where instruction semantics are available but weakly expressed in native continuous actions. We introduce \textbf{SAT-Bench}, a fixed-observation counterfactual framework that holds the visual scene and agent state fixed while changing only instruction semantics. Across two LIBERO-based counterfactual splits, Qwen2.5-VL reliably recovers the intended target, but OpenVLA rarely changes its action. Target recovery reaches 100.0\% and 95.8\%, whereas action sensitivity remains only 6.8\% and 7.7\%. Hidden-state, threshold-free, cross-policy, and rollout diagnostics show that the gap is grounded, behavior-relevant, and not a metric artifact. To expose this boundary, we introduce \textbf{VISA}, a lightweight semantic-action interface that translates recovered semantics into ALLOW, DEFER, and target-consistency decisions. VISA reduces invalid-instruction blind execution from 92.7\% to 2.8\% while preserving 94.0\% of normal commands. These findings suggest that embodied language evaluation should test whether parsed instruction semantics reach the action interface.

\end{abstract}

==> sections/01_introduction.tex <==
\section{Introduction}
\label{sec:intro}

Multimodal language-grounding evaluations often ask whether a model identifies the correct object, relation, or instruction state~\citep{goyal2017making,agrawal2018dont,thrush2022winoground,su2024actplan}. Embodied language agents add an action-interface requirement: recovered semantics should affect whether and how an action is exposed. However, a vision-language-action (VLA) policy~\citep{kim2024openvla,octo2024} may recover the requested target and still move toward a plausible object from scene priors, or may parse a prohibited command and still expose an executable motion. We therefore ask an action-boundary question:
\emph{when the world is fixed, does changing instruction semantics change the
native continuous action accordingly?}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/fig1.png}
\caption{
Fixed-observation counterfactual protocol. The observation and agent state are fixed while only the instruction semantics changes.
}
\label{fig:framework}
\end{figure}

We call this interface-level requirement \emph{semantic--action transfer} (SAT): recovered instruction semantics should affect whether and how a native action is exposed. When semantics are recoverable but remain weakly expressed in the policy's native seven-degree-of-freedom (7-DoF) action, we say the policy exhibits a \emph{semantic--action gap} (SAG). To measure this gap, we use a \emph{fixed-observation counterfactual protocol}: holding the observation and agent state fixed, we change only instruction semantics and test whether the exposed native action changes accordingly. Figure~\ref{fig:framework} illustrates this protocol, which separates \emph{semantic availability} from \emph{semantic control of action}. This distinction is the central thesis of the paper: semantic availability is not semantic action control, so embodied language evaluation should measure semantic-to-action transfer rather than only semantic parsing or task success.

This paper makes this action-boundary problem measurable in two steps: first through a benchmark protocol for diagnosing semantic--action transfer, and then through an interface that exposes action-boundary decisions. We introduce \textsc{SAT-Bench} (\emph{Semantic--Action Transfer Benchmark}), a fixed-observation benchmark protocol spanning target-name changes, relation-defined targets, invalid commands, prohibitions, and paraphrase controls. Across these interventions, we observe a consistent semantic--action gap. On LIBERO~\citep{liu2023libero} target-name and pixel-grounded relation swaps, Qwen2.5-VL~\citep{bai2025qwen25vl} recovers the intended target in 100.0\% and 95.8\% of cases, yet OpenVLA action sensitivity, measured by paraphrase-calibrated native action changes, is only 6.8\% and 7.7\%, respectively. Additional probes, threshold-free analyses, attribution tests, and short-horizon rollouts rule out external-probe, threshold, and grounding-only explanations. The same boundary appears for non-executable language, where invalid or prohibited instructions can still trigger blind native execution.

These diagnostics motivate an explicit semantic-action interface: recovered semantics should not only be readable, but should determine whether a native action is allowed, deferred, or flagged before exposure. We therefore introduce \method{} (\emph{Verifiable Interface for Semantic Action}), a lightweight interface that converts recovered semantics into action-exposure decisions. \method{} extracts a compact instruction-conditioned schema, checks admissibility, passes through valid native actions, defers invalid ones, and flags allowed actions that contradict the recovered target. The goal is not to build a new low-level controller, but to expose and regulate the semantic-action boundary. Empirically, \method{} reduces invalid-instruction blind execution from 92.7\% to 2.8\%, preserves 94.0\% of normal commands, and surfaces wrong-target or ambiguous native actions before execution. In short, \method{} operationalizes the paper's thesis at the action boundary: recovered semantics should determine when to allow, defer, or flag native action exposure.

Our contributions are four-fold:
\begin{itemize}[topsep=0pt, itemsep=2pt, parsep=0pt, leftmargin=1em]
\item a formulation of \emph{semantic--action transfer} and \emph{semantic--action gaps} as interface-level requirements for embodied language grounding;
\item \textsc{SAT-Bench}, a release-ready fixed-observation counterfactual benchmark protocol with prompt transformations, ActCheck labels, policy adapters, and evaluation scripts;
\item diagnostic evidence that named and relation-defined targets can be recoverable externally and inside OpenVLA representations while remaining weakly transferred to native actions;
\item \method{}, a schema-based semantic-action interface that converts recovered semantics into allow, defer, and target-consistency decisions without replacing the low-level policy.
\end{itemize} 

==> sections/02_related_work.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Grounded language evaluation, counterfactuals, and probing.}
Multimodal grounding work tests whether models recover intended objects, relations, or scene states from language and perception. Counterfactual and contrastive evaluations further ask whether predictions rely on intended semantic variables rather than dataset priors or superficial correlations~\citep{goyal2017making,agrawal2018dont,thrush2022winoground}. Related embodied and procedural benchmarks study planning, grounding, scene consistency, and robustness under semantic perturbations~\citep{su2024actplan,chakraborty2025heal}. We target a narrower action-interface question: holding the observation and agent state fixed, does changing only the instruction induce the corresponding change in the exposed action? We also draw on representation probing, which tests whether task-relevant information is present in intermediate states~\citep{alain2016understanding,hewitt2019structural,belinkov2022survey}; in our setting, probing helps separate absent semantic recovery from failed transfer into action~\citep{zhang2025knowing}.

\paragraph{Embodied language agents and VLA benchmarks.}
Recent embodied foundation models connect visual observations, language instructions, and actions through imitation learning, multimodal pretraining, and large robot datasets~\citep{brohan2022rt1,driess2023palme,zitkovich2023rt2,oneill2023openx}. OpenVLA and Octo provide open-source VLA policies that enable controlled inspection of language-conditioned action behavior~\citep{kim2024openvla,octo2024}, while LIBERO offers language-conditioned manipulation tasks for transfer evaluation~\citep{liu2023libero}. These works primarily evaluate task success, generalization, or imitation quality. Our focus is complementary: we use native actions as a readout of grounded-language transfer rather than as the sole target of control optimization.

\paragraph{Invalid instructions, structured semantics, and action interfaces.}
A related line of work studies whether embodied agents can reject false-premise commands, infeasible requests, unsafe instructions, or scene-task inconsistencies~\citep{hsieh2025dowhat,chakraborty2025heal,son2025safel}. High-level language-to-robot systems combine language reasoning with affordances, feedback, or programmatic primitives to improve executable planning~\citep{ahn2022saycan,huang2022inner,liang2022code}. Robotic language understanding has long used structured semantic representations to connect commands with objects, relations, actions, and constraints~\citep{tellex2011understanding,thomason2015learning,thomason2019improving}; modern VLMs such as Qwen2.5-VL provide image-conditioned parsing and grounding~\citep{bai2025qwen25vl}. VISA builds on this interface view, but uses schemas for evaluation and exposure decisions: whether recovered semantics should allow, defer, or flag an action.

==> sections/03_experiment_setup.tex <==
\section{Semantic--Action Transfer Framework}
\label{sec:framework}

We formalize embodied instruction following as an action-interface problem with two separable requirements: the relevant semantic state must be recoverable, and the exposed continuous action must be controlled by that state. The goal is not to optimize robot motion, but to evaluate whether recovered semantics reach the native action interface. We first define semantic--action transfer under fixed observations, then introduce \textsc{SAT-Bench} interventions, and finally define measurements for action sensitivity, non-execution, and target consistency.

\subsection{Interface Requirement under Fixed Observations}
\label{sec:problem_formulation}

Let $o$ denote the visual observation together with the robot state, $x$ a natural-language instruction, and $a=f(o,x)$ the native continuous action predicted by a VLA policy. We study an interface-level requirement: if the instruction semantics change while the world state is fixed, the exposed action should change in the corresponding semantic direction.

A counterfactual instruction $x'=C(x)$ changes the requested semantics while keeping $o$ fixed, yielding $a'=f(o,x')$. The fixed-observation design is a measurement protocol rather than the definition of the failure itself. If both the image and the instruction change, an action difference could be caused by language, visual features, object layout, or scene priors. By holding $o$ fixed, the protocol isolates the instruction-conditioned component of action selection.

This formulation separates two questions often conflated in embodied evaluation: whether the semantics are recoverable from $(o,x)$, and whether the native action head expresses those semantics. We call the desired interface property semantic--action transfer (SAT). When semantic recovery is high but action control is weak, the policy exhibits a semantic--action gap (SAG). Thus, SAG is not a claim that the model lacks language understanding; it is a behavioral claim about where recovered semantics fail to reach the action boundary.

\subsection{\textsc{SAT-Bench} Interventions}
\label{sec:setup_splits}

\textsc{SAT-Bench} instantiates the fixed-observation protocol through controlled semantic interventions over the instruction while the observation and robot state remain fixed. We use
\begin{equation}
C \in \{C_{\mathrm{name}}, C_{\mathrm{rel}}, C_{\mathrm{invalid}}, C_{\mathrm{neg}}, C_{\mathrm{para}}\},
\end{equation}
where each intervention probes a distinct semantic-to-action property.

$C_{\mathrm{name}}$ replaces the explicitly named target while the scene is fixed, e.g., ``pick up the black bowl'' becomes ``pick up the ramekin,'' testing whether target semantics control the next action. $C_{\mathrm{rel}}$ removes the target name and specifies the target through a spatial relation to an anchor object, testing whether grounded relational semantics reach the same action boundary. $C_{\mathrm{invalid}}$ converts executable commands into blank, impossible, ambiguous, or unsupported instructions, testing whether non-executable semantics inhibit action exposure. $C_{\mathrm{neg}}$ constructs prohibited commands such as \texttt{do\_not}, \texttt{avoid}, \texttt{leave\_alone}, and \texttt{except}, testing whether language can block an otherwise plausible action. $C_{\mathrm{para}}$ produces semantically equivalent paraphrases, which calibrate wording-induced action variation.

Together, these interventions cover the three interface behaviors needed for semantic--action transfer: redirecting actions, inhibiting inadmissible actions, and calibrating action variation induced by wording alone.

\subsection{Measurement Stack}
\label{sec:setup_action_sensitivity}

We use a three-part measurement stack. \textbf{Action-sensitivity metrics} test whether a semantic intervention changes the native action beyond wording-induced variation. \textbf{Non-execution metrics} test whether non-executable semantics suppress action exposure. \textbf{Target-consistency metrics} test whether an allowed action points toward the recovered target rather than a competing target. Together, these measurements separate three interface questions: whether actions change, whether invalid actions are withheld, and whether exposed actions are semantically directed.

\paragraph{Action-sensitivity metrics.}
For target-changing interventions, we measure native action sensitivity using a normalized action difference:
\begin{equation}
    D(a,a') = \left\| (a-a') \oslash \sigma_a \right\|_2,
\end{equation}
where $\sigma_a$ is the policy-specific action standard deviation. An action is counted as sensitive if $D(a,a')>\tau$, with $\tau$ calibrated as the 95th percentile of semantically equivalent paraphrase controls. We use $\tau_{\mathrm{OpenVLA}}=2.2851$ for OpenVLA and $\tau_{\mathrm{Octo}}=2.063$ for Octo-small-1.5.

Given a semantic availability signal $\mathrm{SemSens}$, we quantify the semantic--action gap as the mismatch between semantic availability and action sensitivity:
\begin{equation}
    \mathrm{SAG} = \mathrm{SemSens} - \mathrm{ActionSens}.
\end{equation}
For target-name swaps, $\mathrm{SemSens}$ is schema sensitivity; for oracle relation swaps, $\mathrm{SemSens}=1$; and for pixel-grounded relation swaps, $\mathrm{SemSens}$ is grounding accuracy over all examples or $1$ on the grounding-correct subset. To avoid making the diagnosis depend on a single cutoff, we also report target-vs-control AUC over the full action-delta distribution.

\paragraph{Non-execution metrics.}
For inadmissible instructions, the desired interface behavior is non-execution rather than a different target-directed motion. Let $a_{\mathrm{orig}}=f(o,x)$ be the action under the original valid instruction and $a_{\mathrm{inv}}=f(o,x_{\mathrm{invalid}})$ the action under an invalid perturbation. We define
\begin{equation}
\begin{aligned}
\mathrm{BlindExec} &= \mathbb{I}\!\left[D(a_{\mathrm{orig}},a_{\mathrm{inv}})<\tau\right],\\
\mathrm{ActionInhib} &= 1-\mathrm{BlindExec}.
\end{aligned}
\end{equation}
Blind execution measures whether an invalid instruction still exposes a native action close to the original executable command. Action inhibition measures whether non-executable semantics suppress that exposure. At the schema level, an invalid instruction is rejected if the execution decision is a safe deferral such as \texttt{ask}, \texttt{hold}, \texttt{abort}, or \texttt{target-not-found}. We report invalid safe deferral together with normal-command pass rate so that a trivial all-stop system cannot score well by refusing every instruction.

\paragraph{Target-consistency metrics.}
\label{sec:setup_actcheck}
Action sensitivity only asks whether the action changes; it does not determine whether the new action is directed toward the intended target. We therefore define \actcheck{}, a target-consistency diagnostic. Let $p_e$ be the end-effector position, $p_t$ the intended target position, $p_w$ a competing wrong or original target, and $v=a_{1:3}$ the translational action. We compute
\begin{equation}
 c_t=\cos(v,p_t-p_e), \qquad c_w=\cos(v,p_w-p_e).
\end{equation}
With margin $\delta_{\mathrm{ac}}$, the action is target-aligned if $c_t-c_w>\delta_{\mathrm{ac}}$, wrong-target if $c_w-c_t>\delta_{\mathrm{ac}}$, and ambiguous otherwise.

Crossing this label with schema correctness yields \emph{schema--action attribution}, which separates grounding failures from semantic-to-action transfer failures. A wrong schema with a wrong action is primarily a recoverability failure; a correct schema with a wrong or ambiguous action is an interface-transfer failure; and a correct schema with an aligned action is the desired case.

\subsection{From Diagnostics to \method{}}
\label{sec:why_interface}

These measurements localize failures at the action boundary. If semantics are unrecoverable, the bottleneck is perception or language understanding; if semantics are recoverable but actions do not change, the bottleneck is semantic-to-action transfer; if invalid instructions still expose actions, the bottleneck is admissibility; and if allowed actions point to the wrong target, the bottleneck is target consistency. This motivates \method{}: an interface that converts recovered semantics into allow, defer, and target-consistency decisions without replacing the low-level policy.

==> sections/04_diagnostic_results.tex <==
\section{Diagnostic Evidence for the Semantic--Action Gap}
\label{sec:diagnostic_results}

We evaluate the semantic--action gap through three diagnostic questions:
whether recoverable semantics control native actions, whether the gap survives
artifact checks, and whether the same boundary appears when semantics should
inhibit action exposure.

Unless otherwise specified, the action policy is OpenVLA and the schema or
grounding probe is Qwen2.5-VL-7B-Instruct. We additionally evaluate
OpenVLA-LIBERO90 and Octo-small-1.5, and use BridgeData V2 as a real-robot
instruction-change diagnostic. The semantic probe measures recoverability only;
it does not modify native policy actions. The full diagnostic pipeline is shown
in Appendix~\ref{app:diagnostic_pipeline}.
\label{sec:diag_setup}

\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.98}

\begingroup
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}

\begin{tabularx}{0.98\textwidth}{@{}
>{\raggedright\arraybackslash}X
>{\raggedright\arraybackslash}X
>{\raggedright\arraybackslash}X
r r r r r
@{}}
\toprule
\rowcolor{HeaderBg}
\textbf{\rule{0pt}{2.5ex}Policy}
& \textbf{Domain}
& \textbf{Intervention}
& $\boldsymbol{N}$
& \textbf{Sem.}
& \textbf{Act.}
& \textbf{Gap}
& \textbf{ActCheck} \\
\midrule
\rowcolor{GapBg}
OpenVLA base      & LIBERO        & target-name    & 600 & 100.0 & 6.8  & \textbf{93.2} & -- \\
OpenVLA-LIBERO90  & LIBERO        & target-name    & 600 & 100.0 & 5.7  & 94.3 & -- \\
Octo-small-1.5    & LIBERO        & target-name    & 600 & 100.0 & 42.7 & 57.3 & -- \\
\rowcolor{GapBg}
OpenVLA base      & LIBERO        & pixel relation & 600 & 95.8  & 7.7  & \textbf{88.1} & 45.5 \\
Octo-small-1.5    & LIBERO        & pixel relation & 600 & 95.8  & 37.5 & 58.3 & 42.8 \\
Octo-small-1.5    & BridgeData V2 & target/task    & 165 & 100.0 & 66.1 & 33.9 & limited \\
\bottomrule
\end{tabularx}

\endgroup

\caption{Semantic-to-action transfer across policies and domains. Gap is Sem. minus Act.; values except $N$ are percentages.}
\label{tab:cross_policy_diagnostics}
\end{table*}

\subsection{Recoverable Semantics Weakly Control Native Actions}
\label{sec:diag_main_gap}

The first diagnostic question is whether target semantics, once recoverable,
actually control the native action interface. In target-name swaps, the schema
target changes in 100.0\% of cases, but OpenVLA actions are sensitive in only
6.8\%. This shows that even an explicit target change does not reliably reach
the native action. In pixel-grounded relation swaps, Qwen2.5-VL grounds the
target correctly in 95.8\% of cases, while OpenVLA action sensitivity remains
only 7.7\%. This setting is especially diagnostic because the target name is
absent from the instruction and must be recovered from the image and spatial
relation.

Figure~\ref{fig:main_gap_chart} visualizes the main OpenVLA gap, and
Table~\ref{tab:cross_policy_diagnostics} extends the comparison across policies
and domains. OpenVLA-LIBERO90 shows the same pattern on LIBERO target-name
swaps. Octo-small-1.5 and BridgeData V2 are more responsive, but still leave
residual gaps between semantic signal and action sensitivity. These results show
that semantic--action transfer is a graded axis rather than an OpenVLA-specific
binary failure.

\begin{figure}[!htbp]
\centering
\includegraphics[width=0.92\linewidth]{figures/fig4_main_gap_bar.pdf}
\caption{Main semantic--action gap on OpenVLA counterfactuals. Grounded target semantics are available, but the native action rarely changes accordingly.}
\label{fig:main_gap_chart}
\end{figure}

\textbf{Takeaway.}
Recovered target semantics are available, but they are weakly transferred to the
native action interface. Thus, the failure is not semantic recovery
alone, but semantic-to-action transfer.

\subsection{Ruling Out Artifact Explanations}
\label{sec:diag_threshold_quadrant}

We next test whether the gap can be explained away by simpler
alternatives: external-probe artifacts, threshold choice, grounding failure, or
one-step diagnostics with no behavioral relevance.

\paragraph{Internal availability.}
\label{sec:hidden_probe_main}
A natural alternative explanation is that only the external Qwen probe recovers
the target, while the action policy itself lacks the relevant information. We
therefore train linear probes on OpenVLA action-prompt hidden states.
Table~\ref{tab:hidden_probe_main} shows that named targets are readable from
OpenVLA representations, and that the same pattern holds for relation-defined
targets whose names are absent from the instruction. In the full pixel-relation
condition, the hidden-state probe recovers the grounded target with schema
sensitivity 1.000, while decoded action sensitivity remains 0.094. On an
image-dependent subset where language-only or shuffled-image controls fail,
schema sensitivity remains 1.000 but action sensitivity falls to 0.060. Thus,
the relevant target information can be readable inside the action policy even
when decoded actions remain weakly controlled by it. A preliminary activation
patching check is reported in Appendix~\ref{app:activation_patching}; we treat
the probes as semantic-availability evidence rather than as a causal repair.

\begin{table}[!htbp]
\centering
\scriptsize
\setlength{\tabcolsep}{2.4pt}
\renewcommand{\arraystretch}{0.90}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{llrrr}
\toprule
Probe setting & Condition/subset & Sem. sens. & Act. sens. & Gap \\
\midrule
Target-name & full & 1.000 & 0.078 & 0.922 \\
Target-name & mask-target & 0.728 & 0.078 & 0.650 \\
Target-name & random-label & 0.061 & 0.078 & -0.017 \\
Pixel relation & full image+relation & 1.000 & 0.094 & 0.906 \\
Pixel relation & image-dependent & 1.000 & 0.060 & 0.940 \\
Pixel relation & language-only & 0.594 & 0.094 & 0.500 \\
Pixel relation & shuffled-image & 0.656 & 0.094 & 0.561 \\
Pixel relation & random-label & 0.067 & 0.094 & -0.028 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{
OpenVLA hidden-state probe results. Semantics are linearly readable, while decoded actions remain weakly sensitive.
}
\label{tab:hidden_probe_main}
\end{table}

\paragraph{Metric robustness.}
We test whether the gap is an artifact of the paraphrase-calibrated action
threshold. Threshold-free comparisons show that OpenVLA target-name and
pixel-relation swaps remain only weakly separable from paraphrase controls, with
AUCs of 57.3 and 58.3. Spatially separated subsets lead to the same conclusion,
with angle-separated results in Appendix~\ref{app:angle_separated}. In
contrast, BridgeData V2 with Octo reaches AUC 92.9
(Table~\ref{tab:cross_policy_diagnostics}), showing that the metric detects instruction-conditioned action changes when they exist.

\paragraph{Schema--action attribution.}
We also test whether the gap is merely a grounding failure. On the pixel-grounded
relation split, Table~\ref{tab:schema_action_quadrant} crosses schema correctness
with \actcheck{} target-consistency labels. Only 4.2\% of examples fall into
schema-wrong regions, whereas 44.0\% have a correct schema target but a wrong or
ambiguous native action. This places many failures after grounding: the intended
target has been recovered, but the exposed action is not target-consistent.
Qualitative ActCheck examples are provided in Appendix~\ref{app:actcheck_cases}.

\begin{table}[H]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}

\begingroup
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}

\begin{tabularx}{\linewidth}{@{}
>{\raggedright\arraybackslash}X
rr
@{}}
\toprule
\rowcolor{HeaderBg}
\textbf{\rule{0pt}{2.4ex}Schema/action case}
& \textbf{Count}
& \textbf{Rate} \\
\midrule
Correct target + aligned action & 311 & 51.8 \\
\rowcolor{GapBg}
Correct target + wrong/ambig. action & \textbf{264} & \textbf{44.0} \\
Wrong target + aligned action & 16 & 2.7 \\
Wrong target + wrong/ambig. action & 9 & 1.5 \\
\bottomrule
\end{tabularx}

\endgroup

\caption{Schema--action attribution on pixel-grounded relation examples.}
\label{tab:schema_action_quadrant}
\end{table}

\paragraph{Short-horizon behavior relevance.}
\label{sec:robustness_diagnostics}
A final concern is that one-step action diagnostics may not matter for later
behavior. We evaluate 300 paired OpenVLA-LIBERO90 rollouts from identical initial
states for $K=20$ policy steps. Raw counterfactual instructions do not reliably
redirect the trajectory by themselves; aggregate target-approach effects remain
mixed (Appendix~G). However, first-step ActCheck labels strongly stratify later
behavior. Target-aligned first actions lead to significantly
higher final and integrated counterfactual-target
preference than ambiguous or wrong-target first
actions, with full rollout statistics in Appendix~\ref{app:actcheck_predictive_rollout_300}. We therefore do not claim that
first-step actions determine task success; instead, the rollout study validates
ActCheck as a short-horizon predictive diagnostic.


\textbf{Takeaway.}
The semantic--action gap is not explained by external probing, threshold choice,
or grounding failure alone. Target information can be readable inside OpenVLA
and behavior-relevant under ActCheck, yet decoded actions remain weakly
controlled by the semantics.

\subsection{Action Inhibition Reveals the Same Boundary}
\label{sec:diag_negation}

The final diagnostic question is whether semantic--action transfer is limited to
target redirection, or whether the same boundary appears when semantics should
inhibit action exposure. For invalid or prohibited instructions, the relevant
semantic requirement is not to move toward a different object, but to avoid
exposing an executable native action.

The invalid-instruction diagnostic shows that OpenVLA often keeps exposing
target-directed actions when execution should be deferred. OpenVLA blindly
executes 92.7\% of templated invalid instructions. Negation and prohibition show
the same boundary under different wording: on 800 Octo negation/prohibition
variants, Octo inhibits only 29.8\% of prohibited commands, leaving 70.2\% blind
execution (Figure~\ref{fig:negation_stress_main}). The 300 non-template invalid
examples are independently audited in Appendix~\ref{app:hard_invalid_audit}, with
all examples labeled as requiring deferral. Direct binary VLM gating remains
brittle to linguistic form, whereas schema-level admissibility checks provide a
clearer interface signal.

\begin{figure}[H]
\centering
\includegraphics[width=0.94\linewidth]{figures/fig5_negation_stress_bar.pdf}
\caption{
Non-executable language stress test on prohibited commands.
}
\label{fig:negation_stress_main}
\end{figure}

These results extend the semantic--action gap beyond target selection. In
target-changing counterfactuals, recovered semantics fail to redirect the native
action; in invalid and prohibited instructions, recovered non-executable
semantics fail to inhibit action exposure.

\textbf{Takeaway.}
Semantic--action failures also appear when the correct behavior is non-execution:
invalid or prohibited instructions can still expose plausible native actions.
This motivates an interface that can gate action exposure before execution.

Overall, these diagnostics localize failures at the action boundary: semantics
can be recoverable externally and internally, yet fail to redirect native actions,
inhibit invalid commands, or guarantee target-consistent exposure.
Section~\ref{sec:visa} turns this diagnosis into an interface design that
converts recovered semantics into allow, defer, and target-consistency decisions.

\FloatBarrier

==> sections/05_visa.tex <==
\section{\method{}: A Semantic-Action Interface for Action Exposure}
\label{sec:visa}

Section~\ref{sec:diagnostic_results} localizes semantic--action failures at the
action boundary: recovered semantics may fail to redirect native actions, invalid
instructions may still expose executable motions, and target-correct schemas may
still yield wrong-target or ambiguous actions. \method{} responds to these
failures with an explicit semantic-action interface. It exposes recovered
instruction semantics, decides whether execution is admissible, passes through
valid native actions, defers inadmissible instructions, and flags
target-inconsistent actions before execution. Table~\ref{tab:visa_mapping}
summarizes this mapping from diagnostics to interface decisions.

\begin{table}[!htbp]
\centering
\small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabularx}{\linewidth}{@{}
>{\raggedright\arraybackslash}X
>{\raggedright\arraybackslash}X
>{\centering\arraybackslash}p{0.17\linewidth}
@{}}
\toprule
\textbf{Diagnostic failure} & \textbf{\method{} mechanism} & \textbf{Decision} \\
\midrule
Invalid or prohibited instruction exposes action
& Admissibility gate
& \textsc{DEFER} \\
Valid instruction with admissible native action
& Native-action pass-through
& \textsc{ALLOW} \\
Correct schema but wrong/ambiguous action
& \actcheck{} target-consistency check
& \textsc{FLAG} \\
Recoverable target with weak native transfer
& Schema-level repair signal
& Inspect / \textsc{FLAG} \\
\bottomrule
\end{tabularx}
\caption{
How \method{} maps semantic--action diagnostics to action-exposure decisions.
}
\label{tab:visa_mapping}
\end{table}

\method{} is lightweight because it does not replace the policy, synthesize
grasps, or plan trajectories; it is interpretable because its decisions are
mediated by an auditable schema and deterministic checks. Figure~\ref{fig:visa_interface}
summarizes the interface: schema extraction makes the recovered semantic state
explicit, the admissibility gate decides whether a native action should be
exposed, and \actcheck{} flags allowed actions that contradict the recovered target.

\begin{figure}[!htbp]
\centering
\includegraphics[width=0.92\linewidth,trim=0 2 0 2,clip]{figures/fig3_visa_interface.png}
\caption{
\method{} semantic-action interface: schema extraction, admissibility checking, and action exposure.
}
\label{fig:visa_interface}
\end{figure}

\subsection{Interface Components: Schema, Gate, and \actcheck{}}
\label{sec:visa_components}

\textbf{Schema extraction.}
For a task family $\tau$, \method{} extracts a task-specific schema
\begin{equation}
    s_\tau = g_\theta(o,x;K_\tau), \qquad K_\tau \subseteq K,
\end{equation}
where $K_\tau$ selects the keys needed by the task. We use a compact schema
\begin{equation}
    s_\tau=(t,e,A^+,A^-,u,d,r),
\end{equation}
where $t$ is the target, $e$ is target existence, $A^+$ and $A^-$ are allowed
and blocked symbolic action sets, $u$ is the next symbolic action, $d$ is the
execution decision, and $r$ is a reason. The action vocabulary is a small set,
\begin{equation}
\begin{aligned}
A_\tau \subseteq \{&\texttt{move\_to\_target},\texttt{grasp},\texttt{open},\texttt{close},\\
&\texttt{place},\texttt{hold},\texttt{ask},\texttt{abort}\}.
\end{aligned}
\end{equation}
Task families select different key subsets, but all schemas expose the
interface variables needed for action exposure: target state, admissibility,
blocked actions, next symbolic action, and reason.

\textbf{Admissibility gate.}
The checker enforces instruction-conditioned constraints over the schema. Blank
commands should not infer a task from scene priors, impossible-target commands
should not execute target-directed actions, and prohibited commands should not
execute blocked actions. The interface policy is
\begin{equation}
\pi_{\mathrm{VISA}}(o,x)=
\begin{cases}
(f(o,x),\textsc{ALLOW}), & \text{if } \mathrm{admissible}(s_\tau),\\
(\varnothing,\textsc{DEFER}(r)), & \text{otherwise}.
\end{cases}
\end{equation}
Thus, allowed native actions are passed through unchanged, while inadmissible
instructions defer execution and expose a reason rather than an action.

\textbf{\actcheck{}.}
The gate decides whether an action may be exposed; \actcheck{} decides
whether an allowed action is target-consistent. Using the target recovered in
$s_\tau$, \actcheck{} applies the target-consistency test from
Section~\ref{sec:setup_actcheck}. Wrong-target or ambiguous allowed actions are
surfaced as \textsc{FLAG} decisions before execution. This makes
target-inconsistent behavior inspectable rather than hiding it behind a single
action-delta score.

\subsection{Exposure Decisions, Not Control}
\label{sec:visa_application}

\method{} is an interface-level mechanism, not a low-level controller. It does
not synthesize grasps, plan trajectories, verify collision risk, or certify
long-horizon task success. Its intervention target is action exposure: whether
to pass through a native action, defer execution, or flag a target-inconsistent
action.

This scope matches the diagnostics in Section~\ref{sec:diagnostic_results} and
determines the evaluation in Section~\ref{sec:visa_eval}. We evaluate safe
deferral, normal-command pass-through, \actcheck{} flags, and repair signals as
action-boundary decisions rather than task-completion claims. In this sense,
\method{} operationalizes semantic--action transfer as an auditable
allow--defer--flag interface between recovered semantics and native actions.

==> sections/06_visa_evaluation.tex <==
\FloatBarrier
\section{Evaluating \method{} as an Action-Exposure Interface}
\label{sec:visa_eval}

Section~\ref{sec:visa} defines \method{} as an action-exposure interface rather
than a low-level controller. We therefore evaluate whether it makes the intended
interface decisions: defer inadmissible instructions, preserve admissible native
actions, flag target-inconsistent actions, and expose repair signals without
claiming task-level control.

\subsection{Deferring Invalid Commands while Preserving Valid Ones}
\label{sec:visa_safe_deferral}

The non-execution diagnostics in Section~\ref{sec:diag_negation} show that
native policies can expose target-directed actions even when execution should be
deferred. \method{} directly addresses this failure by separating semantic
extraction from admissibility checking. On templated invalid instructions, it
raises safe deferral to 97.2\%, reducing blind execution from 92.7\% to 2.8\%.

Negation and prohibition show the same pattern under different wording. Octo
inhibits only 29.8\% of prohibited commands, and a direct binary Qwen gate safely
defers 36.5\%. \method{} instead extracts blocked-action and admissibility fields
and applies deterministic checks, reaching 100.0\% safe deferral with 0.0\%
blind allow.

Safe deferral alone is not sufficient: a trivial system could avoid blind
execution by refusing every command. Figure~\ref{fig:visa_safety_utility}
therefore reports a balanced semantic-interface score, defined as the worse of
invalid safe deferral and normal-command pass-through. \method{} scores 94.0,
compared with 40.7 for Direct Qwen, 7.3 for Raw OpenVLA, and 0.0 for all-stop.
Thus, the improvement is not an all-stop artifact: \method{} converts invalid
semantics into \textsc{DEFER} decisions while preserving useful native actions on
admissible commands.

\begin{figure}[t]
\centering
\includegraphics[width=0.90\linewidth]{figures/fig6_visa_safety_utility_scorecard.pdf}
\caption{
Deferral--utility balance. The score is the minimum of invalid safe deferral and normal pass-through.
}
\label{fig:visa_safety_utility}
\end{figure}

\subsection{Flagging Target-Inconsistent Native Actions}
\label{sec:visa_target_flags}

The diagnostic results also show that action sensitivity does not imply target
consistency. On pixel-grounded relation examples, OpenVLA is target-aligned in
54.5\% of cases and wrong or ambiguous in 45.5\%. Using the recovered schema
target, \actcheck{} turns these wrong-target or ambiguous allowed actions into
explicit pre-execution flags.

This is the interface counterpart of schema--action attribution. When the schema
is correct but the native action is inconsistent, the failure should not be
hidden behind a single action-delta score; it should be surfaced before
execution. \actcheck{} does not certify task success, but it exposes
target-inconsistent native actions as \textsc{FLAG} decisions before execution.

\subsection{Repair Signals Are Not Controller Claims}
\label{sec:visa_repair_signal}

Correct schema targets can also define target-consistent directional candidates
when the native action is wrong or ambiguous. We use this only as an
interface-level repair signal: it shows that the recovered semantic state
contains information that could support a target-consistent alternative, but it
does not synthesize a full manipulation trajectory or certify task success
(Appendix~\ref{app:repair_proxy}).

Together, these results show that \method{} improves action-boundary decisions:
it can allow admissible native actions, defer inadmissible instructions, flag
target-inconsistent actions, and expose repair signals without replacing the
low-level policy.

==> sections/07_conclusion.tex <==
%\section{Conclusion}

%Semantic availability is not action control. We identify the semantic--action gap as a grounded-language transfer failure at the action interface: instruction semantics can be recoverable while native continuous actions remain weakly controlled by them. To measure this gap, we introduced a fixed-observation counterfactual framework and prompt-transformation data strategy that hold the world fixed while changing only instruction semantics. Our diagnostics show that named and relation-defined targets can be recovered externally and read from OpenVLA representations, yet decoded actions remain weakly sensitive; non-executable instructions reveal the same boundary through blind execution. VISA operationalizes the framework as a lightweight interpretable semantic-action interface, converting recovered semantics into \textsc{allow}, \textsc{defer}, and target-consistency decisions without replacing the low-level policy. Embodied language grounding should therefore report whether recovered instruction semantics reach the action interface, not only whether they can be parsed.

\section{Conclusion}
Semantic availability is not action control. We identify the semantic--action gap
as a transfer failure: instruction semantics can be recoverable while native
actions remain weakly controlled. SAT-Bench measures this gap with
fixed-observation counterfactuals that change only instruction semantics. Our
diagnostics show that named and relation-defined targets can be recovered
externally and read from OpenVLA representations, yet decoded actions remain
weakly sensitive; invalid instructions reveal the same boundary through blind
execution. VISA turns this distinction into ALLOW/DEFER/flag decisions, so
embodied grounding should measure semantic-to-action transfer rather than
semantic recovery alone.

==> sections/07_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

These results reframe embodied language evaluation as an interface question. Grounding tests ask whether a model recovers the referent; we ask whether that recovered state controls exposed action. Hidden-state probes show that named and relation-defined targets are readable inside OpenVLA while decoded actions remain weakly sensitive, making the gap a semantic-to-action transfer bottleneck rather than an external-probe artifact.

The scope is diagnostic: policy/domain results show a graded axis, and ActCheck target-preference analyses connect one-step signals to K=20 behavior, but neither replaces task-success evaluation. VISA is an auditable allow/defer/flag interface, not a controller. We therefore report task success with semantic sensitivity, target consistency, and non-execution.


==> sections/09_limitations.tex <==
% \section*{Limitations}

% \hua{Let's make the limitations to be 1-2 paragraph, you can summarize some points to make it shorter.}
% \paragraph{Benchmark and embodiment scope.}
% Our experiments are concentrated in LIBERO-style tabletop manipulation settings. This provides a controlled and reproducible environment for fixed-observation counterfactual evaluation, but it does not establish that the same quantitative gaps will hold across all robot embodiments, real-world deployments, or non-manipulation domains. We include additional checks with OpenVLA-LIBERO90, Octo-small-1.5, and BridgeData V2, and Octo reduces but does not eliminate the semantic--action gap. The BridgeData V2 target/task-change split uses instruction changes from the first public TFDS shard without object-level metadata, so it should be interpreted as a real-robot instruction-change diagnostic rather than a strict object-grounded target-swap benchmark. A broader policy suite is still needed to characterize how architecture, training data, action representation, embodiment, and fine-tuning affect semantic--action transfer.

% \paragraph{Action metrics, uncertainty, and horizon.}
% Our main action-sensitivity metric compares continuous actions using paraphrase-calibrated thresholds, and we add threshold-free AUC analyses to reduce dependence on a single cutoff. These metrics still do not replace full long-horizon instruction-following evaluation. Relation-defined counterfactuals, spatial controls, target-consistency checks, qualitative cases, and 100 paired $K=20$ rollouts reduce the concern that the result is only a first-action artifact. The aggregate rollout evidence is still mixed because the paired improvement confidence interval crosses zero, although ActCheck labels significantly stratify target preference. Our conclusion is therefore not that one-step metrics determine task success, but that they expose a measurable transfer bottleneck between recovered semantics and native actions.

% \paragraph{Hidden-state probes and causal claims.}
% Linear hidden-state probes show that target identity is readable from OpenVLA action-prompt representations, including named-target and relation-defined settings, while random-label and degraded-input controls are weaker. This is evidence of semantic availability, not a complete causal proof that the action head ignores semantics. Our preliminary activation patching experiment has limited effect on decoded actions, suggesting a representation-to-action bottleneck, but a broader causal intervention study would be needed to fully characterize how the decoder uses intermediate information.

% \paragraph{Visual grounding, schemas, and invalid-instruction coverage.}
% The pixel-grounded relation split tests whether a VLM can infer relation-defined targets from images when the target name is absent from the instruction, but it remains within a finite LIBERO-style object vocabulary and controlled tabletop relations. VISA also depends on the quality of the schema generator: incorrect grounding, ambiguous references, poor target-existence judgments, or inconsistent schema fields can lead to incorrect allow or defer decisions. Our invalid, non-template, and negation/prohibition stress tests cover multiple controlled forms, but they are still constructed diagnostic sets rather than a fully human-authored instruction distribution.

% \paragraph{Verification scope and post-hoc interface design.}
% \actcheck{} verifies whether the translational component of a native action is directionally more consistent with the intended target than with a competing wrong or original target. It does not check grasp feasibility, collision risk, contact dynamics, rotation, gripper state, phase transitions, or long-horizon task completion. VISA is evaluated as a post-hoc diagnostic, gating, and verification layer rather than an end-to-end trained controller. It can measure and partially guard semantic--action transfer failures, but it cannot by itself solve perception, planning, grasp synthesis, closed-loop manipulation, or physical safety. The appropriate operating point may depend on deployment risk, task reversibility, and tolerance for false blocks.
%\section*{Limitations}

%Our experiments are mainly concentrated in LIBERO-style tabletop manipulation settings, which provide a controlled and reproducible testbed for fixed-observation counterfactual evaluation but do not establish that the same quantitative semantic--action gaps will hold across all embodiments, real-world deployments, or non-manipulation domains. We include additional checks with OpenVLA-LIBERO90, Octo-small-1.5, and BridgeData V2; Octo reduces but does not eliminate the gap. The BridgeData V2 target/task-change split is based on instruction changes from the first public TFDS shard and lacks object-level metadata, so it should be interpreted as a real-robot instruction-change diagnostic rather than a strict object-grounded target-swap benchmark. A broader policy suite is still needed to characterize how architecture, training data, action representation, embodiment, and fine-tuning affect semantic--action transfer. Our action-sensitivity metric compares continuous actions using paraphrase-calibrated thresholds, supplemented by threshold-free AUC analyses, but these metrics do not replace full long-horizon instruction-following evaluation. Relation-defined counterfactuals, spatial controls, target-consistency checks, qualitative cases, and 100 paired $K=20$ rollouts reduce the concern that the result is only a first-action artifact; however, the aggregate rollout evidence remains mixed because the paired improvement confidence interval crosses zero, even though ActCheck labels significantly stratify target preference.

%Our hidden-state probes show that target identity is readable from OpenVLA action-prompt representations in both named-target and relation-defined settings, while random-label and degraded-input controls are weaker. This supports semantic availability, but it is not a complete causal proof that the action head ignores semantics. Preliminary activation patching has limited effect on decoded actions, suggesting a representation-to-action bottleneck, but broader causal interventions are needed to fully characterize decoder usage. Similarly, the pixel-grounded relation split tests whether a VLM can infer relation-defined targets from images when the target name is absent, but it remains limited to a finite LIBERO-style object vocabulary and controlled tabletop relations. VISA also depends on schema-generator quality: incorrect grounding, ambiguous references, poor target-existence judgments, or inconsistent schema fields can lead to incorrect allow or defer decisions. Our invalid, non-template, and negation/prohibition stress tests cover multiple controlled forms, but they are not a fully human-authored instruction distribution. Finally, \actcheck{} only verifies whether the translational component of a native action is directionally more consistent with the intended target than with a competing wrong or original target; it does not check grasp feasibility, collision risk, contact dynamics, rotation, gripper state, phase transitions, or long-horizon task completion. VISA should therefore be viewed as a post-hoc diagnostic, gating, and verification layer rather than an end-to-end controller: it can measure and partially guard semantic--action transfer failures, but it does not by itself solve perception, planning, grasp synthesis, closed-loop manipulation, or physical safety.

\section*{Limitations}

Our experiments focus on LIBERO-style tabletop manipulation, which provides a controlled setting for fixed-observation counterfactual evaluation but does not establish that the same quantitative gaps hold across all embodiments, real-world deployments, or non-manipulation domains. We include additional checks with OpenVLA-LIBERO90, Octo-small-1.5, and BridgeData V2, but BridgeData V2 lacks object-level metadata and should be interpreted as a real-robot instruction-change diagnostic rather than a strict object-grounded target-swap benchmark. Our action-sensitivity metrics use paraphrase-calibrated thresholds and threshold-free AUC analyses, but they do not replace full long-horizon instruction-following evaluation. The paired K = 20 rollouts and ActCheck analyses reduce the concern that the
results are only first-action artifacts: first-step target-consistency labels
significantly predict short-horizon target preference. However, aggregate raw
counterfactual rollouts do not constitute a task-success evaluation; our claim
is therefore about a measurable semantic-to-action transfer bottleneck, not
full manipulation success.

Our hidden-state probes show that target information is readable from OpenVLA action-prompt representations, but probing is not a complete causal proof that the action head ignores semantics. Preliminary activation patching has limited effect, and broader causal interventions are needed to characterize how decoded actions use intermediate representations. VISA also depends on schema quality: incorrect grounding, ambiguous references, poor target-existence judgments, or inconsistent schema fields can lead to incorrect allow or defer decisions. Finally, \actcheck{} only verifies whether the translational action is directionally more consistent with the intended target than with a competing target; it does not check grasp feasibility, collision risk, contact dynamics, rotation, gripper state, phase transitions, or long-horizon completion. VISA should therefore be viewed as a post-hoc semantic-action interface, not an end-to-end controller or complete robot safety system.

==> sections/10_ethics.tex <==
\section*{Ethics Statement}
\label{sec:ethics}

This work studies failure modes in embodied vision-language-action agents and proposes diagnostic tools for identifying when instruction semantics are not faithfully reflected in robot actions. The intended use is to improve evaluation, transparency, and safety by exposing plausible but semantically inappropriate actions before they are executed.

VISA and \actcheck{} should not be interpreted as complete robot safety systems. They are post-hoc diagnostic and action-interface mechanisms that can block or flag some semantic--action failures, but they do not verify physical safety, grasp feasibility, collision risk, contact dynamics, long-horizon task completion, or recovery behavior. Real-world deployment would require additional safeguards, including conservative fail-safe control, hardware-level safety validation, calibrated uncertainty handling, human override mechanisms, and domain-specific risk assessment.

A potential risk of this work is false confidence: a system that passes VISA-style checks may still behave unsafely due to perception errors, distribution shift, ambiguous instructions, or low-level control failures. We therefore present VISA as a diagnostic and verification interface for studying semantic--action transfer, not as a deployable controller or a sufficient safeguard for real-world robots.
